PlanFitting: Personalized Exercise Planning with Large Language Model-driven Conversational Agent

Creating personalized and actionable exercise plans often requires iteration with experts, which can be costly and inaccessible to many individuals. This work explores the capabilities of Large Language Models (LLMs) in addressing these challenges. We present PlanFitting, an LLM-driven conversational agent that assists users in creating and refining personalized weekly exercise plans. By engaging users in free-form conversations, PlanFitting helps elicit users' goals, availabilities, and potential obstacles, and enables individuals to generate personalized exercise plans aligned with established exercise guidelines. Our study -- involving a user study, intrinsic evaluation, and expert evaluation -- demonstrated PlanFitting's ability to guide users to create tailored, actionable, and evidence-based plans. We discuss future design opportunities for LLM-driven conversational agents to create plans that better comply with exercise principles and accommodate personal constraints.

==> figures/interface.tex <==
\begin{teaserfigure}
    \centering
    \includegraphics[width=\textwidth]{figures/fig_interface.pdf}
    \caption{Key screen of the \system{} system. As the user chats with the system on the chat panel (right), \system{} leads the conversation and collects the user's personal constraints (\circledigit{A}), recommends exercise types based on the provided constraints (\circledigit{B}), and sets up personalized plan in the form of if-then rules (\circledigit{C}).}
    \Description{A key screen of the PlanFitting system, which consists of a chat panel on the right side and a dashboard on the left side}
    \label{fig:interface}
\end{teaserfigure}

==> figures/survey_planner.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=.55\textwidth]{figures/fig_survey_planner.pdf}
    \caption{Survey results from our exploratory study with expert planners.}
    \Description{This figure displays the survey results from our exploratory study with expert planners, represented as points stacked within the grid box. It has frequency, intensity, time, and type as sub-categories.}
    \label{fig:survey_planner}
\end{figure*}

==> figures/survey_user.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_survey_user.pdf}
    \caption{Survey results from our exploratory study with participants. The results for each subset of (a) are calculated as the mean score of its sub-questionnaires, and the rightmost points denote the responses with 7-point on average.}
    \Description{This figure displays the survey results from our exploratory study with participants, represented as points stacked within the grid box. It has technology acceptance model, personalization, and actionability as sub-categories.}
    \label{fig:survey_user}
    \labelphantom{fig:survey_user:tam}
    \labelphantom{fig:survey_user:personalization}
    \labelphantom{fig:survey_user:actionability}

\end{figure*}
